Using Invalid Instruments on Purpose: Focused Moment Selection and Averaging for GMM

In finite samples, the use of a slightly endogenous but highly relevant instrument can reduce mean-squared error (MSE). Building on this observation, I propose a novel moment selection procedure for GMM -- the Focused Moment Selection Criterion (FMSC) -- in which moment conditions are chosen not based on their validity but on the MSE of their associated estimator of a user-specified target parameter. The FMSC mimics the situation faced by an applied researcher who begins with a set of relatively mild "baseline" assumptions and must decide whether to impose any of a collection of stronger but more controversial "suspect" assumptions. When the (correctly specified) baseline moment conditions identify the model, the FMSC provides an asymptotically unbiased estimator of asymptotic MSE, allowing us to select over the suspect moment conditions. I go on to show how the framework used to derive the FMSC can address the problem of inference post-moment selection. Treating post-selection estimators as a special case of moment-averaging, in which estimators based on different moment sets are given data-dependent weights, I propose simulation-based procedures for inference that can be applied to a variety of formal and informal moment-selection and averaging procedures. Both the FMSC and confidence interval procedures perform well in simulations. I conclude with an empirical example examining the effect of instrument selection on the estimated relationship between malaria and income per capita.

==> AdditionalSimulations/LimitSimResults/c_1equal_OLSvsIV.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $94$ & $94$ & $96$ & $96$ & $94$ & $90$\\ 
$\pi^2\;\;\;$ $0.2$ & $95$ & $95$ & $95$ & $94$ & $91$ & $92$\\ 
$0.3$ & $95$ & $96$ & $94$ & $93$ & $93$ & $94$\\ 
$0.4$ & $96$ & $95$ & $93$ & $93$ & $95$ & $95$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $90$ & $90$ & $91$ & $89$ & $85$ & $81$\\ 
$\pi^2\;\;\;$ $0.2$ & $91$ & $91$ & $89$ & $85$ & $84$ & $86$\\ 
$0.3$ & $92$ & $91$ & $88$ & $86$ & $87$ & $90$\\ 
$0.4$ & $92$ & $90$ & $87$ & $87$ & $90$ & $91$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $86$ & $84$ & $77$ & $70$ & $68$ & $68$\\ 
$\pi^2\;\;\;$ $0.2$ & $86$ & $83$ & $75$ & $72$ & $72$ & $77$\\ 
$0.3$ & $86$ & $81$ & $74$ & $73$ & $78$ & $81$\\ 
$0.4$ & $86$ & $79$ & $75$ & $77$ & $81$ & $81$\\ 
 \hline 
 \end{tabular}

==> AdditionalSimulations/LimitSimResults/c_1equal_chooseIVs.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $96$ & $95$ & $94$ & $94$ & $94$ & $95$\\ 
$\gamma^2\;\;\;$ $0.2$ & $96$ & $96$ & $95$ & $93$ & $93$ & $94$\\ 
$0.3$ & $95$ & $96$ & $95$ & $93$ & $93$ & $92$\\ 
$0.4$ & $95$ & $95$ & $96$ & $94$ & $92$ & $91$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $92$ & $90$ & $88$ & $88$ & $89$ & $91$\\ 
$\gamma^2\;\;\;$ $0.2$ & $92$ & $91$ & $88$ & $86$ & $87$ & $89$\\ 
$0.3$ & $92$ & $91$ & $89$ & $86$ & $86$ & $87$\\ 
$0.4$ & $91$ & $91$ & $90$ & $86$ & $84$ & $85$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $84$ & $81$ & $76$ & $77$ & $80$ & $81$\\ 
$\gamma^2\;\;\;$ $0.2$ & $86$ & $82$ & $75$ & $74$ & $77$ & $80$\\ 
$0.3$ & $86$ & $82$ & $76$ & $72$ & $73$ & $78$\\ 
$0.4$ & $86$ & $83$ & $77$ & $72$ & $72$ & $75$\\ 
 \hline 
 \end{tabular}

==> AdditionalSimulations/LimitSimResults/c_2equal_OLSvsIV.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $98$ & $98$ & $98$ & $98$ & $99$ & $98$\\ 
$\pi^2\;\;\;$ $0.2$ & $98$ & $98$ & $98$ & $98$ & $98$ & $98$\\ 
$0.3$ & $98$ & $98$ & $98$ & $98$ & $98$ & $98$\\ 
$0.4$ & $98$ & $98$ & $98$ & $98$ & $98$ & $98$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $96$ & $96$ & $97$ & $97$ & $97$ & $96$\\ 
$\pi^2\;\;\;$ $0.2$ & $96$ & $97$ & $97$ & $97$ & $96$ & $95$\\ 
$0.3$ & $97$ & $97$ & $97$ & $96$ & $95$ & $96$\\ 
$0.4$ & $97$ & $97$ & $96$ & $95$ & $96$ & $97$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $93$ & $94$ & $94$ & $94$ & $94$ & $93$\\ 
$\pi^2\;\;\;$ $0.2$ & $94$ & $94$ & $94$ & $93$ & $92$ & $90$\\ 
$0.3$ & $95$ & $94$ & $93$ & $91$ & $90$ & $92$\\ 
$0.4$ & $95$ & $94$ & $92$ & $90$ & $92$ & $93$\\ 
 \hline 
 \end{tabular}

==> AdditionalSimulations/LimitSimResults/c_2equal_chooseIVs.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $99$ & $99$ & $98$ & $98$ & $98$ & $98$\\ 
$\gamma^2\;\;\;$ $0.2$ & $98$ & $98$ & $98$ & $98$ & $98$ & $97$\\ 
$0.3$ & $98$ & $98$ & $98$ & $98$ & $98$ & $98$\\ 
$0.4$ & $98$ & $98$ & $98$ & $98$ & $98$ & $98$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $98$ & $97$ & $96$ & $95$ & $95$ & $96$\\ 
$\gamma^2\;\;\;$ $0.2$ & $97$ & $97$ & $97$ & $96$ & $95$ & $95$\\ 
$0.3$ & $97$ & $97$ & $97$ & $96$ & $96$ & $95$\\ 
$0.4$ & $97$ & $97$ & $97$ & $97$ & $96$ & $96$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $95$ & $94$ & $91$ & $90$ & $91$ & $92$\\ 
$\gamma^2\;\;\;$ $0.2$ & $95$ & $94$ & $93$ & $91$ & $90$ & $91$\\ 
$0.3$ & $95$ & $94$ & $94$ & $93$ & $91$ & $90$\\ 
$0.4$ & $94$ & $94$ & $94$ & $93$ & $92$ & $90$\\ 
 \hline 
 \end{tabular}

==> AdditionalSimulations/LimitSimResults/c_2narrowtau_OLSvsIV.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $99$ & $99$ & $99$ & $99$ & $99$ & $99$\\ 
$\pi^2\;\;\;$ $0.2$ & $99$ & $99$ & $99$ & $99$ & $99$ & $99$\\ 
$0.3$ & $99$ & $99$ & $99$ & $99$ & $99$ & $99$\\ 
$0.4$ & $99$ & $99$ & $99$ & $99$ & $99$ & $99$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $98$ & $98$ & $98$ & $98$ & $99$ & $98$\\ 
$\pi^2\;\;\;$ $0.2$ & $98$ & $98$ & $98$ & $98$ & $98$ & $98$\\ 
$0.3$ & $98$ & $98$ & $98$ & $98$ & $98$ & $98$\\ 
$0.4$ & $98$ & $98$ & $98$ & $98$ & $98$ & $98$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $96$ & $96$ & $97$ & $97$ & $97$ & $96$\\ 
$\pi^2\;\;\;$ $0.2$ & $97$ & $97$ & $97$ & $97$ & $96$ & $95$\\ 
$0.3$ & $97$ & $97$ & $97$ & $96$ & $95$ & $95$\\ 
$0.4$ & $97$ & $97$ & $96$ & $95$ & $96$ & $96$\\ 
 \hline 
 \end{tabular}

==> AdditionalSimulations/LimitSimResults/c_2narrowtau_chooseIVs.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $99$ & $99$ & $99$ & $99$ & $99$ & $99$\\ 
$\gamma^2\;\;\;$ $0.2$ & $99$ & $99$ & $99$ & $99$ & $99$ & $99$\\ 
$0.3$ & $99$ & $99$ & $99$ & $99$ & $99$ & $99$\\ 
$0.4$ & $99$ & $99$ & $99$ & $99$ & $99$ & $99$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $99$ & $98$ & $98$ & $98$ & $98$ & $98$\\ 
$\gamma^2\;\;\;$ $0.2$ & $98$ & $98$ & $98$ & $98$ & $98$ & $97$\\ 
$0.3$ & $98$ & $98$ & $98$ & $98$ & $98$ & $98$\\ 
$0.4$ & $98$ & $98$ & $98$ & $98$ & $98$ & $98$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $97$ & $97$ & $96$ & $95$ & $95$ & $96$\\ 
$\gamma^2\;\;\;$ $0.2$ & $97$ & $97$ & $97$ & $96$ & $95$ & $95$\\ 
$0.3$ & $97$ & $97$ & $97$ & $97$ & $96$ & $95$\\ 
$0.4$ & $97$ & $97$ & $97$ & $97$ & $96$ & $96$\\ 
 \hline 
 \end{tabular}

==> AdditionalSimulations/LimitSimResults/w_1equal_OLSvsIV.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $ 96$ & $ 96$ & $ 97$ & $ 99$ & $101$ & $103$\\ 
$\pi^2\;\;\;$ $0.2$ & $ 97$ & $ 98$ & $100$ & $104$ & $107$ & $109$\\ 
$0.3$ & $ 97$ & $ 99$ & $103$ & $107$ & $109$ & $107$\\ 
$0.4$ & $ 98$ & $100$ & $105$ & $108$ & $107$ & $104$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $ 93$ & $ 94$ & $ 95$ & $ 99$ & $103$ & $106$\\ 
$\pi^2\;\;\;$ $0.2$ & $ 95$ & $ 96$ & $100$ & $105$ & $110$ & $110$\\ 
$0.3$ & $ 97$ & $ 98$ & $105$ & $108$ & $110$ & $108$\\ 
$0.4$ & $ 97$ & $101$ & $107$ & $109$ & $106$ & $102$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $ 90$ & $ 90$ & $ 94$ & $ 99$ & $104$ & $109$\\ 
$\pi^2\;\;\;$ $0.2$ & $ 93$ & $ 97$ & $102$ & $108$ & $111$ & $113$\\ 
$0.3$ & $ 96$ & $100$ & $106$ & $109$ & $110$ & $107$\\ 
$0.4$ & $ 97$ & $101$ & $108$ & $109$ & $106$ & $103$\\ 
 \hline 
 \end{tabular}

==> AdditionalSimulations/LimitSimResults/w_1equal_chooseIVs.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $ 99$ & $100$ & $104$ & $106$ & $107$ & $104$\\ 
$\gamma^2\;\;\;$ $0.2$ & $ 98$ & $ 99$ & $103$ & $106$ & $108$ & $109$\\ 
$0.3$ & $ 97$ & $ 98$ & $101$ & $105$ & $109$ & $109$\\ 
$0.4$ & $ 97$ & $ 98$ & $100$ & $103$ & $106$ & $109$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $ 98$ & $100$ & $105$ & $107$ & $106$ & $104$\\ 
$\gamma^2\;\;\;$ $0.2$ & $ 97$ & $ 99$ & $103$ & $107$ & $110$ & $108$\\ 
$0.3$ & $ 96$ & $ 97$ & $101$ & $106$ & $110$ & $110$\\ 
$0.4$ & $ 96$ & $ 97$ & $101$ & $105$ & $108$ & $110$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $ 98$ & $101$ & $105$ & $107$ & $106$ & $103$\\ 
$\gamma^2\;\;\;$ $0.2$ & $ 98$ & $ 99$ & $104$ & $109$ & $110$ & $108$\\ 
$0.3$ & $ 96$ & $ 96$ & $103$ & $107$ & $110$ & $111$\\ 
$0.4$ & $ 94$ & $ 95$ & $102$ & $106$ & $111$ & $112$\\ 
 \hline 
 \end{tabular}

==> AdditionalSimulations/LimitSimResults/w_2equal_OLSvsIV.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $121$ & $121$ & $123$ & $125$ & $129$ & $131$\\ 
$\pi^2\;\;\;$ $0.2$ & $123$ & $124$ & $127$ & $129$ & $132$ & $134$\\ 
$0.3$ & $124$ & $125$ & $128$ & $130$ & $132$ & $132$\\ 
$0.4$ & $124$ & $125$ & $128$ & $129$ & $129$ & $128$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $131$ & $130$ & $134$ & $136$ & $140$ & $142$\\ 
$\pi^2\;\;\;$ $0.2$ & $131$ & $132$ & $136$ & $139$ & $141$ & $142$\\ 
$0.3$ & $132$ & $133$ & $136$ & $138$ & $139$ & $139$\\ 
$0.4$ & $133$ & $134$ & $135$ & $136$ & $136$ & $134$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $148$ & $150$ & $150$ & $153$ & $158$ & $160$\\ 
$\pi^2\;\;\;$ $0.2$ & $148$ & $149$ & $151$ & $155$ & $156$ & $158$\\ 
$0.3$ & $147$ & $149$ & $150$ & $152$ & $153$ & $151$\\ 
$0.4$ & $146$ & $148$ & $149$ & $149$ & $148$ & $144$\\ 
 \hline 
 \end{tabular}

==> AdditionalSimulations/LimitSimResults/w_2equal_chooseIVs.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $124$ & $125$ & $126$ & $126$ & $126$ & $126$\\ 
$\gamma^2\;\;\;$ $0.2$ & $124$ & $125$ & $127$ & $129$ & $130$ & $130$\\ 
$0.3$ & $122$ & $124$ & $127$ & $129$ & $131$ & $132$\\ 
$0.4$ & $123$ & $124$ & $126$ & $129$ & $131$ & $133$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $132$ & $132$ & $132$ & $133$ & $133$ & $132$\\ 
$\gamma^2\;\;\;$ $0.2$ & $132$ & $133$ & $135$ & $136$ & $138$ & $137$\\ 
$0.3$ & $132$ & $132$ & $135$ & $137$ & $140$ & $140$\\ 
$0.4$ & $132$ & $132$ & $135$ & $137$ & $140$ & $141$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $145$ & $145$ & $145$ & $145$ & $144$ & $142$\\ 
$\gamma^2\;\;\;$ $0.2$ & $147$ & $148$ & $150$ & $150$ & $151$ & $150$\\ 
$0.3$ & $147$ & $148$ & $151$ & $153$ & $154$ & $154$\\ 
$0.4$ & $148$ & $148$ & $152$ & $154$ & $155$ & $157$\\ 
 \hline 
 \end{tabular}

==> AdditionalSimulations/LimitSimResults/w_2narrowtau_OLSvsIV.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $132$ & $132$ & $134$ & $136$ & $140$ & $143$\\ 
$\pi^2\;\;\;$ $0.2$ & $133$ & $134$ & $138$ & $142$ & $145$ & $147$\\ 
$0.3$ & $135$ & $136$ & $140$ & $143$ & $145$ & $145$\\ 
$0.4$ & $136$ & $137$ & $141$ & $142$ & $143$ & $142$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $143$ & $144$ & $146$ & $149$ & $152$ & $157$\\ 
$\pi^2\;\;\;$ $0.2$ & $145$ & $146$ & $150$ & $154$ & $157$ & $159$\\ 
$0.3$ & $146$ & $148$ & $152$ & $155$ & $156$ & $157$\\ 
$0.4$ & $147$ & $150$ & $152$ & $154$ & $153$ & $152$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $165$ & $166$ & $168$ & $173$ & $177$ & $179$\\ 
$\pi^2\;\;\;$ $0.2$ & $168$ & $168$ & $173$ & $177$ & $180$ & $182$\\ 
$0.3$ & $167$ & $169$ & $173$ & $177$ & $178$ & $177$\\ 
$0.4$ & $168$ & $170$ & $174$ & $174$ & $173$ & $169$\\ 
 \hline 
 \end{tabular}

==> AdditionalSimulations/LimitSimResults/w_2narrowtau_chooseIVs.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.05$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $136$ & $137$ & $138$ & $139$ & $140$ & $140$\\ 
$\gamma^2\;\;\;$ $0.2$ & $135$ & $137$ & $139$ & $142$ & $143$ & $144$\\ 
$0.3$ & $134$ & $134$ & $138$ & $142$ & $144$ & $145$\\ 
$0.4$ & $133$ & $134$ & $138$ & $141$ & $144$ & $145$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.1$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $148$ & $148$ & $150$ & $150$ & $150$ & $150$\\ 
$\gamma^2\;\;\;$ $0.2$ & $147$ & $147$ & $150$ & $153$ & $155$ & $155$\\ 
$0.3$ & $145$ & $147$ & $150$ & $153$ & $156$ & $158$\\ 
$0.4$ & $145$ & $146$ & $150$ & $153$ & $156$ & $158$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\tau$} \\ 
 $\alpha = 0.2$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ 
 \hline$0.1$ & $168$ & $168$ & $169$ & $170$ & $170$ & $168$\\ 
$\gamma^2\;\;\;$ $0.2$ & $167$ & $169$ & $171$ & $174$ & $176$ & $175$\\ 
$0.3$ & $167$ & $168$ & $171$ & $176$ & $178$ & $179$\\ 
$0.4$ & $167$ & $167$ & $170$ & $175$ & $178$ & $181$\\ 
 \hline 
 \end{tabular}

==> SimulationChooseIVs/Results/coverage_FMSC_2step.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $89$ & $88$ & $88$ & $87$ & $89$ & $89$\\ 
$0.2$ & $90$ & $88$ & $87$ & $86$ & $88$ & $89$\\ 
$\gamma\quad$$0.3$ & $91$ & $89$ & $87$ & $85$ & $86$ & $88$\\ 
$0.4$ & $91$ & $91$ & $87$ & $84$ & $83$ & $87$\\ 
$0.5$ & $92$ & $91$ & $88$ & $84$ & $82$ & $84$\\ 
$0.6$ & $92$ & $92$ & $90$ & $85$ & $82$ & $81$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $92$ & $90$ & $90$ & $91$ & $91$ & $91$\\ 
$0.2$ & $92$ & $90$ & $88$ & $89$ & $91$ & $91$\\ 
$\gamma\quad$$0.3$ & $93$ & $90$ & $87$ & $88$ & $90$ & $91$\\ 
$0.4$ & $94$ & $92$ & $86$ & $84$ & $88$ & $90$\\ 
$0.5$ & $94$ & $93$ & $87$ & $83$ & $84$ & $89$\\ 
$0.6$ & $94$ & $93$ & $89$ & $82$ & $82$ & $86$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $95$ & $93$ & $92$ & $92$ & $92$ & $92$\\ 
$0.2$ & $96$ & $91$ & $92$ & $91$ & $92$ & $93$\\ 
$\gamma\quad$$0.3$ & $96$ & $89$ & $92$ & $92$ & $92$ & $93$\\ 
$0.4$ & $96$ & $89$ & $90$ & $91$ & $92$ & $93$\\ 
$0.5$ & $96$ & $90$ & $87$ & $91$ & $91$ & $92$\\ 
$0.6$ & $95$ & $92$ & $83$ & $91$ & $91$ & $92$\\ 
 \hline 
 \end{tabular}

==> SimulationChooseIVs/Results/coverage_FMSC_naive.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $80$ & $78$ & $77$ & $79$ & $81$ & $82$\\ 
$0.2$ & $79$ & $75$ & $73$ & $74$ & $79$ & $81$\\ 
$\gamma\quad$$0.3$ & $79$ & $72$ & $66$ & $67$ & $73$ & $78$\\ 
$0.4$ & $78$ & $71$ & $62$ & $59$ & $66$ & $75$\\ 
$0.5$ & $78$ & $68$ & $57$ & $52$ & $57$ & $67$\\ 
$0.6$ & $77$ & $68$ & $54$ & $47$ & $50$ & $60$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $84$ & $82$ & $84$ & $86$ & $86$ & $86$\\ 
$0.2$ & $83$ & $77$ & $78$ & $84$ & $87$ & $86$\\ 
$\gamma\quad$$0.3$ & $82$ & $74$ & $71$ & $79$ & $85$ & $86$\\ 
$0.4$ & $82$ & $71$ & $63$ & $71$ & $82$ & $86$\\ 
$0.5$ & $81$ & $69$ & $56$ & $62$ & $76$ & $84$\\ 
$0.6$ & $81$ & $66$ & $51$ & $52$ & $69$ & $81$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $89$ & $88$ & $89$ & $89$ & $90$ & $90$\\ 
$0.2$ & $87$ & $84$ & $90$ & $90$ & $90$ & $90$\\ 
$\gamma\quad$$0.3$ & $86$ & $77$ & $89$ & $90$ & $90$ & $90$\\ 
$0.4$ & $85$ & $67$ & $88$ & $89$ & $90$ & $90$\\ 
$0.5$ & $84$ & $59$ & $84$ & $90$ & $90$ & $89$\\ 
$0.6$ & $83$ & $52$ & $77$ & $89$ & $90$ & $90$\\ 
 \hline 
 \end{tabular}

==> SimulationChooseIVs/Results/coverage_Valid.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $83$ & $83$ & $83$ & $82$ & $83$ & $83$\\ 
$0.2$ & $83$ & $83$ & $83$ & $83$ & $84$ & $83$\\ 
$\gamma\quad$$0.3$ & $83$ & $82$ & $83$ & $83$ & $83$ & $83$\\ 
$0.4$ & $82$ & $83$ & $84$ & $83$ & $83$ & $84$\\ 
$0.5$ & $84$ & $83$ & $83$ & $83$ & $83$ & $83$\\ 
$0.6$ & $83$ & $83$ & $83$ & $83$ & $82$ & $82$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $86$ & $87$ & $87$ & $87$ & $86$ & $86$\\ 
$0.2$ & $86$ & $86$ & $86$ & $86$ & $87$ & $86$\\ 
$\gamma\quad$$0.3$ & $86$ & $86$ & $87$ & $87$ & $87$ & $87$\\ 
$0.4$ & $86$ & $87$ & $86$ & $86$ & $87$ & $87$\\ 
$0.5$ & $87$ & $87$ & $86$ & $86$ & $86$ & $86$\\ 
$0.6$ & $87$ & $86$ & $86$ & $87$ & $86$ & $87$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $90$ & $89$ & $89$ & $89$ & $90$ & $90$\\ 
$0.2$ & $89$ & $90$ & $90$ & $90$ & $90$ & $90$\\ 
$\gamma\quad$$0.3$ & $89$ & $90$ & $90$ & $90$ & $90$ & $90$\\ 
$0.4$ & $89$ & $90$ & $90$ & $89$ & $90$ & $90$\\ 
$0.5$ & $90$ & $90$ & $90$ & $90$ & $90$ & $89$\\ 
$0.6$ & $89$ & $89$ & $89$ & $90$ & $90$ & $90$\\ 
 \hline 
 \end{tabular}

==> SimulationChooseIVs/Results/coverage_posFMSC_2step.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $89$ & $88$ & $88$ & $87$ & $89$ & $89$\\ 
$0.2$ & $90$ & $88$ & $87$ & $86$ & $88$ & $89$\\ 
$\gamma\quad$$0.3$ & $91$ & $89$ & $87$ & $85$ & $86$ & $88$\\ 
$0.4$ & $91$ & $90$ & $87$ & $84$ & $83$ & $87$\\ 
$0.5$ & $92$ & $91$ & $88$ & $84$ & $82$ & $84$\\ 
$0.6$ & $92$ & $92$ & $90$ & $85$ & $82$ & $81$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $92$ & $90$ & $90$ & $91$ & $91$ & $91$\\ 
$0.2$ & $92$ & $90$ & $88$ & $89$ & $91$ & $91$\\ 
$\gamma\quad$$0.3$ & $93$ & $90$ & $87$ & $88$ & $90$ & $91$\\ 
$0.4$ & $94$ & $92$ & $86$ & $84$ & $88$ & $90$\\ 
$0.5$ & $94$ & $93$ & $87$ & $83$ & $84$ & $89$\\ 
$0.6$ & $94$ & $93$ & $89$ & $82$ & $82$ & $86$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $95$ & $93$ & $92$ & $92$ & $92$ & $92$\\ 
$0.2$ & $96$ & $91$ & $92$ & $91$ & $92$ & $93$\\ 
$\gamma\quad$$0.3$ & $96$ & $89$ & $92$ & $92$ & $92$ & $93$\\ 
$0.4$ & $96$ & $89$ & $90$ & $91$ & $92$ & $93$\\ 
$0.5$ & $96$ & $90$ & $87$ & $91$ & $91$ & $92$\\ 
$0.6$ & $95$ & $92$ & $83$ & $91$ & $91$ & $92$\\ 
 \hline 
 \end{tabular}

==> SimulationChooseIVs/Results/width_FMSC_2step.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $20$ & $18$ & $18$ & $17$ & $17$ & $19$\\ 
$0.2$ & $20$ & $18$ & $17$ & $16$ & $16$ & $16$\\ 
$\gamma\quad$$0.3$ & $21$ & $17$ & $15$ & $14$ & $14$ & $17$\\ 
$0.4$ & $21$ & $17$ & $13$ & $13$ & $13$ & $15$\\ 
$0.5$ & $22$ & $16$ & $13$ & $12$ & $12$ & $13$\\ 
$0.6$ & $22$ & $17$ & $13$ & $10$ & $10$ & $12$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $20$ & $18$ & $16$ & $15$ & $14$ & $14$\\ 
$0.2$ & $22$ & $17$ & $15$ & $13$ & $12$ & $14$\\ 
$\gamma\quad$$0.3$ & $22$ & $16$ & $13$ & $12$ & $12$ & $14$\\ 
$0.4$ & $21$ & $16$ & $11$ & $10$ & $10$ & $14$\\ 
$0.5$ & $21$ & $15$ & $11$ & $9$ & $9$ & $12$\\ 
$0.6$ & $21$ & $15$ & $11$ & $8$ & $8$ & $11$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $22$ & $17$ & $13$ & $10$ & $8$ & $7$\\ 
$0.2$ & $22$ & $15$ & $10$ & $7$ & $6$ & $9$\\ 
$\gamma\quad$$0.3$ & $21$ & $13$ & $8$ & $6$ & $7$ & $12$\\ 
$0.4$ & $20$ & $13$ & $7$ & $6$ & $7$ & $11$\\ 
$0.5$ & $19$ & $13$ & $8$ & $6$ & $6$ & $9$\\ 
$0.6$ & $20$ & $13$ & $8$ & $5$ & $6$ & $8$\\ 
 \hline 
 \end{tabular}

==> SimulationChooseIVs/Results/width_posFMSC_2step.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $19$ & $18$ & $17$ & $17$ & $17$ & $18$\\ 
$0.2$ & $20$ & $18$ & $16$ & $16$ & $15$ & $16$\\ 
$\gamma\quad$$0.3$ & $21$ & $17$ & $15$ & $14$ & $14$ & $16$\\ 
$0.4$ & $21$ & $17$ & $13$ & $13$ & $13$ & $14$\\ 
$0.5$ & $22$ & $16$ & $13$ & $12$ & $12$ & $13$\\ 
$0.6$ & $22$ & $17$ & $13$ & $10$ & $10$ & $12$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $20$ & $17$ & $16$ & $15$ & $14$ & $14$\\ 
$0.2$ & $21$ & $17$ & $15$ & $13$ & $12$ & $14$\\ 
$\gamma\quad$$0.3$ & $21$ & $16$ & $12$ & $12$ & $12$ & $14$\\ 
$0.4$ & $21$ & $15$ & $11$ & $10$ & $10$ & $14$\\ 
$0.5$ & $21$ & $15$ & $11$ & $9$ & $9$ & $12$\\ 
$0.6$ & $21$ & $15$ & $11$ & $8$ & $8$ & $11$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $21$ & $17$ & $13$ & $10$ & $8$ & $7$\\ 
$0.2$ & $22$ & $15$ & $10$ & $7$ & $6$ & $9$\\ 
$\gamma\quad$$0.3$ & $21$ & $13$ & $8$ & $6$ & $7$ & $12$\\ 
$0.4$ & $20$ & $13$ & $7$ & $6$ & $7$ & $11$\\ 
$0.5$ & $19$ & $13$ & $8$ & $6$ & $6$ & $9$\\ 
$0.6$ & $20$ & $13$ & $8$ & $5$ & $6$ & $8$\\ 
 \hline 
 \end{tabular}

==> SimulationOLSvsIV/Results/coverage_AVG_correct.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $100$ & $100$ & $100$ & $99$ & $98$ & $96$\\ 
$0.2$ & $100$ & $100$ & $100$ & $99$ & $98$ & $96$\\ 
$\pi\quad$$0.3$ & $100$ & $100$ & $99$ & $99$ & $98$ & $95$\\ 
$0.4$ & $99$ & $99$ & $99$ & $98$ & $97$ & $94$\\ 
$0.5$ & $99$ & $99$ & $98$ & $98$ & $96$ & $93$\\ 
$0.6$ & $98$ & $98$ & $98$ & $97$ & $96$ & $93$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $100$ & $100$ & $100$ & $100$ & $99$ & $97$\\ 
$0.2$ & $100$ & $100$ & $100$ & $99$ & $98$ & $95$\\ 
$\pi\quad$$0.3$ & $99$ & $99$ & $99$ & $99$ & $97$ & $94$\\ 
$0.4$ & $99$ & $99$ & $99$ & $98$ & $96$ & $94$\\ 
$0.5$ & $98$ & $99$ & $98$ & $97$ & $95$ & $94$\\ 
$0.6$ & $98$ & $98$ & $97$ & $96$ & $95$ & $95$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $100$ & $100$ & $100$ & $99$ & $98$ & $95$\\ 
$0.2$ & $99$ & $99$ & $99$ & $98$ & $96$ & $94$\\ 
$\pi\quad$$0.3$ & $98$ & $98$ & $98$ & $97$ & $95$ & $97$\\ 
$0.4$ & $98$ & $98$ & $97$ & $96$ & $96$ & $97$\\ 
$0.5$ & $98$ & $98$ & $96$ & $96$ & $97$ & $97$\\ 
$0.6$ & $98$ & $97$ & $96$ & $96$ & $97$ & $96$\\ 
 \hline 
 \end{tabular}

==> SimulationOLSvsIV/Results/coverage_FMSC_correct.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $100$ & $100$ & $99$ & $99$ & $98$ & $97$\\ 
$0.2$ & $99$ & $99$ & $99$ & $99$ & $98$ & $97$\\ 
$\pi\quad$$0.3$ & $99$ & $99$ & $99$ & $99$ & $98$ & $96$\\ 
$0.4$ & $98$ & $98$ & $98$ & $98$ & $98$ & $95$\\ 
$0.5$ & $97$ & $98$ & $98$ & $98$ & $97$ & $94$\\ 
$0.6$ & $97$ & $97$ & $97$ & $97$ & $96$ & $94$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $100$ & $99$ & $99$ & $99$ & $99$ & $98$\\ 
$0.2$ & $99$ & $99$ & $99$ & $99$ & $99$ & $97$\\ 
$\pi\quad$$0.3$ & $98$ & $98$ & $99$ & $99$ & $98$ & $95$\\ 
$0.4$ & $97$ & $97$ & $98$ & $98$ & $97$ & $94$\\ 
$0.5$ & $97$ & $97$ & $98$ & $97$ & $95$ & $95$\\ 
$0.6$ & $97$ & $97$ & $97$ & $96$ & $95$ & $96$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $99$ & $99$ & $99$ & $99$ & $99$ & $96$\\ 
$0.2$ & $97$ & $97$ & $98$ & $99$ & $97$ & $94$\\ 
$\pi\quad$$0.3$ & $96$ & $97$ & $98$ & $97$ & $95$ & $98$\\ 
$0.4$ & $96$ & $97$ & $97$ & $95$ & $98$ & $98$\\ 
$0.5$ & $96$ & $97$ & $96$ & $97$ & $98$ & $98$\\ 
$0.6$ & $96$ & $97$ & $95$ & $97$ & $97$ & $96$\\ 
 \hline 
 \end{tabular}

==> SimulationOLSvsIV/Results/coverage_FMSC_naive.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $88$ & $80$ & $58$ & $30$ & $11$ & $4$\\ 
$0.2$ & $88$ & $79$ & $59$ & $34$ & $15$ & $10$\\ 
$\pi\quad$$0.3$ & $87$ & $81$ & $62$ & $39$ & $25$ & $23$\\ 
$0.4$ & $86$ & $80$ & $66$ & $46$ & $38$ & $43$\\ 
$0.5$ & $86$ & $81$ & $68$ & $56$ & $54$ & $62$\\ 
$0.6$ & $85$ & $81$ & $72$ & $66$ & $67$ & $75$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $88$ & $72$ & $36$ & $10$ & $4$ & $4$\\ 
$0.2$ & $87$ & $74$ & $40$ & $17$ & $13$ & $19$\\ 
$\pi\quad$$0.3$ & $86$ & $74$ & $45$ & $29$ & $32$ & $45$\\ 
$0.4$ & $85$ & $74$ & $51$ & $43$ & $54$ & $70$\\ 
$0.5$ & $85$ & $76$ & $59$ & $57$ & $70$ & $84$\\ 
$0.6$ & $85$ & $78$ & $66$ & $68$ & $81$ & $88$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $87$ & $31$ & $8$ & $12$ & $16$ & $24$\\ 
$0.2$ & $84$ & $35$ & $24$ & $42$ & $62$ & $80$\\ 
$\pi\quad$$0.3$ & $83$ & $42$ & $43$ & $70$ & $87$ & $90$\\ 
$0.4$ & $84$ & $49$ & $62$ & $86$ & $90$ & $90$\\ 
$0.5$ & $84$ & $57$ & $76$ & $89$ & $90$ & $90$\\ 
$0.6$ & $86$ & $66$ & $84$ & $90$ & $90$ & $90$\\ 
 \hline 
 \end{tabular}

==> SimulationOLSvsIV/Results/coverage_TSLS.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $98$ & $98$ & $96$ & $93$ & $89$ & $82$\\ 
$0.2$ & $97$ & $97$ & $95$ & $93$ & $88$ & $83$\\ 
$\pi\quad$$0.3$ & $96$ & $96$ & $94$ & $92$ & $88$ & $85$\\ 
$0.4$ & $94$ & $93$ & $93$ & $91$ & $89$ & $87$\\ 
$0.5$ & $92$ & $92$ & $92$ & $91$ & $90$ & $88$\\ 
$0.6$ & $91$ & $91$ & $90$ & $90$ & $90$ & $88$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $98$ & $98$ & $97$ & $94$ & $89$ & $83$\\ 
$0.2$ & $96$ & $96$ & $95$ & $92$ & $89$ & $85$\\ 
$\pi\quad$$0.3$ & $94$ & $94$ & $93$ & $91$ & $89$ & $87$\\ 
$0.4$ & $92$ & $92$ & $92$ & $91$ & $90$ & $88$\\ 
$0.5$ & $91$ & $91$ & $90$ & $90$ & $89$ & $89$\\ 
$0.6$ & $90$ & $90$ & $90$ & $90$ & $90$ & $89$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $96$ & $96$ & $94$ & $93$ & $90$ & $86$\\ 
$0.2$ & $92$ & $92$ & $91$ & $91$ & $90$ & $89$\\ 
$\pi\quad$$0.3$ & $91$ & $91$ & $91$ & $91$ & $90$ & $90$\\ 
$0.4$ & $90$ & $90$ & $91$ & $90$ & $90$ & $90$\\ 
$0.5$ & $90$ & $90$ & $90$ & $90$ & $90$ & $90$\\ 
$0.6$ & $90$ & $91$ & $90$ & $90$ & $90$ & $90$\\ 
 \hline 
 \end{tabular}

==> SimulationOLSvsIV/Results/width_AVG_correct.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $32$ & $33$ & $33$ & $33$ & $33$ & $33$\\ 
$0.2$ & $33$ & $34$ & $34$ & $34$ & $34$ & $34$\\ 
$\pi\quad$$0.3$ & $34$ & $35$ & $34$ & $34$ & $35$ & $34$\\ 
$0.4$ & $35$ & $35$ & $35$ & $35$ & $34$ & $34$\\ 
$0.5$ & $36$ & $36$ & $35$ & $34$ & $34$ & $33$\\ 
$0.6$ & $36$ & $35$ & $35$ & $33$ & $32$ & $32$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $33$ & $32$ & $32$ & $32$ & $32$ & $33$\\ 
$0.2$ & $34$ & $33$ & $34$ & $33$ & $34$ & $35$\\ 
$\pi\quad$$0.3$ & $35$ & $35$ & $34$ & $35$ & $35$ & $35$\\ 
$0.4$ & $35$ & $35$ & $35$ & $35$ & $35$ & $35$\\ 
$0.5$ & $36$ & $36$ & $35$ & $34$ & $33$ & $33$\\ 
$0.6$ & $36$ & $35$ & $34$ & $32$ & $32$ & $32$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $31$ & $32$ & $33$ & $33$ & $34$ & $35$\\ 
$0.2$ & $33$ & $34$ & $35$ & $36$ & $37$ & $39$\\ 
$\pi\quad$$0.3$ & $35$ & $35$ & $36$ & $36$ & $37$ & $38$\\ 
$0.4$ & $35$ & $35$ & $35$ & $36$ & $36$ & $36$\\ 
$0.5$ & $36$ & $35$ & $34$ & $34$ & $34$ & $31$\\ 
$0.6$ & $36$ & $33$ & $32$ & $32$ & $30$ & $25$\\ 
 \hline 
 \end{tabular}

==> SimulationOLSvsIV/Results/width_FMSC_correct.tex <==
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 50$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $40$ & $41$ & $41$ & $41$ & $42$ & $42$\\ 
$0.2$ & $41$ & $42$ & $42$ & $43$ & $42$ & $42$\\ 
$\pi\quad$$0.3$ & $42$ & $43$ & $43$ & $43$ & $43$ & $43$\\ 
$0.4$ & $43$ & $43$ & $43$ & $43$ & $43$ & $43$\\ 
$0.5$ & $43$ & $42$ & $42$ & $42$ & $42$ & $41$\\ 
$0.6$ & $41$ & $41$ & $40$ & $40$ & $39$ & $38$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 100$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $40$ & $41$ & $41$ & $41$ & $41$ & $42$\\ 
$0.2$ & $42$ & $42$ & $42$ & $42$ & $43$ & $44$\\ 
$\pi\quad$$0.3$ & $43$ & $43$ & $43$ & $44$ & $45$ & $46$\\ 
$0.4$ & $43$ & $43$ & $43$ & $44$ & $44$ & $44$\\ 
$0.5$ & $43$ & $43$ & $42$ & $42$ & $42$ & $42$\\ 
$0.6$ & $42$ & $41$ & $40$ & $39$ & $39$ & $39$\\ 
 \hline 
 \end{tabular}
 
 \vspace{2em} 
 
\begin{tabular}{r|rrrrrr}
\hline\hline
 &\multicolumn{6}{c}{$\rho$} \\ 
 $N = 500$ & $0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$ \\ 
 \hline$0.1$ & $40$ & $41$ & $42$ & $42$ & $43$ & $46$\\ 
$0.2$ & $42$ & $43$ & $45$ & $47$ & $49$ & $51$\\ 
$\pi\quad$$0.3$ & $43$ & $44$ & $46$ & $48$ & $49$ & $49$\\ 
$0.4$ & $43$ & $44$ & $45$ & $46$ & $46$ & $44$\\ 
$0.5$ & $43$ & $43$ & $42$ & $42$ & $39$ & $27$\\ 
$0.6$ & $42$ & $40$ & $39$ & $37$ & $28$ & $20$\\ 
 \hline 
 \end{tabular}
